A new reference catalogue for the very metal-poor Universe: +150 OB stars in Sextans A

Local Group (LG) very metal-poor massive stars are the best proxy for the First Stars of the Universe and fundamental to modelling the evolution of early galaxies. These stars may follow new evolutionary pathways restricted to very low metallicities, such as chemically homogeneous evolution (CHE). However, given the great distance leap needed to reach very metal-poor galaxies of the LG and vicinity, no comprehensive spectroscopic studies have been carried out at metallicities lower than the Small Magellanic Cloud (SMC, Z = 1/5 Z$_{\odot}$) until now. After five observing campaigns at the 10.4-m Gran Telescopio Canarias, we have assembled a low-resolution (R $\sim$ 1000) spectroscopic collection of more than 150 OB stars in the 1/10 Z$_{\odot}$ galaxy Sextans A, increasing by an order of magnitude the number of massive stars known in this galaxy. The catalogue includes 38 BA-type supergiants, 4 red supergiants, and the first candidate 1/10 Z$_{\odot}$ binary systems, CHE sources and systems hosting stripped stars. The sample massive stars mainly overlap the higher concentrations of neutral gas of Sextans A. However, we find some sources in low HI column-density regions. The colour-magnitude diagram of the galaxy presents large dispersion, which suggests uneven, internal extinction in Sextans A. This is the largest catalogue of OB-type stars ever produced at sub-SMC metallicities. This sample constitutes a fundamental first step to unveiling the evolutionary pathways and fates of very metal-poor massive stars, analyzing the dependence of radiation-driven winds with metallicity, and studying binary systems in an environment analogue to the early Universe.

==> AA_Tables/OBcombos_v0.tex <==
\begin{table*}
\centering
\caption{List of the observing blocks and super-observing blocks coadded to generate the final spectrum of each star observed in the MOS1 run.}
\begin{tabular}{ccl}
\hline
\hline
ID & Exposure time (s) & Exposures\\ \hline
\Remark{MOS1.s01} & 26550 & OB02, OB03, OB04, OB05, OB06, OB07, OB10, OB12, OB13\\
\Remark{MOS1.s02} & 26550 & OB02, sOB03(=OB03+OB04), OB05, OB06, OB10, sOB13(= OB12+OB13+OB14) \\
\Remark{MOS1.s03} & 26550 & OB02, OB03, OB04, OB05, OB06, OB07, OB10, OB12, OB13 \\
\Remark{MOS1.s04} & 26550 & OB02, OB03, OB04, OB05, OB06, OB07, OB10, OB12, OB13 \\
\Remark{MOS1.s06} & 26550 & OB02, OB03, OB05, OB06, OB07, OB10, OB12, OB13, OB14 \\
\Remark{MOS1.s07} & 23600 & OB02, OB03, OB04, OB06, OB10, OB12, OB13, OB14 \\
\Remark{MOS1.s08} & 29500 & OB02, OB03, OB04, OB05, OB06, OB07, OB10, OB12, OB13, OB14 \\
\Remark{MOS1.s10} & 32450 & OB02, OB03, OB04, OB05, OB06, OB07, OB09, OB10, OB12, OB13, OB14 \\
\Remark{MOS1.s11} & 32450 & OB02, OB03, OB04, OB05, OB06, OB07, OB10, OB11, OB12, OB13, OB14 \\
\Remark{MOS1.s12} & 26650 & OB02, sOB03(= OB03+OB04), OB05, OB06,OB10, sOB13(= OB12+OB13+OB14) \\
\Remark{MOS1.s13} & 20650 & OB02, OB03, OB04, OB10, OB11, OB12, OB13 \\
\Remark{MOS1.s14} & 29500 & OB02, OB03, OB04, OB06, OB07, OB10, OB11, OB12, OB13, OB14 \\
% \Remark{MOS1.s09} & 26650 & OB02, sOB03(= OB03+OB04), OB05, OB06, OB10, sOB13(= OB12+OB13+OB14) \\
%MOS1.s15 & 20650 & OB02, OB03, OB04, OB10, OB12, OB13, OB14\\
%MOS1.s16 & 32450 & OB02, OB03, OB04, OB05, OB06, OB07, OB09, OB10, OB12, OB13, OB14\\
\hline
\end{tabular}
\label{tab:OBosOB}
\end{table*}

==> AA_Tables/log_LSS2_v0.tex <==
\begin{table*}
\centering
\caption{LSS2 observing log.}
\label{table:lss2_log}
%\begin{threeparttable}
\begin{tabular}{cccccccc}
\hline
\hline
\begin{tabular}[c]{@{}c@{}} Observing \\ block \end{tabular} &
Target & Date & Seeing ('') & Transparency & Moon & Airmass & Exposure time (s)\\
\hline
OB01 & slit-A & 18 Feb 2020 & 1.0 & Clear & Dark & 1.28 - 1.23 & 2806\\
OB02 & slit-A & 18 Feb 2020 & 1.0 & Clear & Dark & 1.19 - 1.20 & 2806\\
OB03 & slit-B & 18 Feb 2020 & 1.3 & Clear & Dark & 1.23 - 1.28 & 2806\\
OB04 & slit-B & 18 Mar 2020 & 0.9 & Phot. & Dark & 1.53 - 1.68 & 2806\\
\hline
\end{tabular}

\begin{tablenotes}%[para,flushleft]
    \begin{flushleft}
        \small
        \textbf{Notes.} Airmass column indicates starting - final airmass of science objects.
    \end{flushleft}
\end{tablenotes}

\end{table*}

==> AA_Tables/log_LSS2_v1.tex <==
\begin{table*}
\centering
\caption{LSS2 observing log.}
\label{table:lss2_log}
%\begin{threeparttable}
\begin{tabular}{ccccccccc}
\hline
\hline
\begin{tabular}[c]{@{}c@{}} Observing \\ block \end{tabular} & Date & Seeing ('') & Slit-width ('') & Transparency & Moon & Airmass & Exposure time (s)\\
\hline
OB01 & 18 Feb 2020 & 1.0 & 1.2 & Clear & Dark & 1.28 - 1.23 & 2806\\
OB02 & 18 Feb 2020 & 1.0 & 1.2 & Clear & Dark & 1.19 - 1.20 & 2806\\
OB03 & 18 Feb 2020 & 1.3 & 1.2 & Clear & Dark & 1.23 - 1.28 & 2806\\
OB04 & 18 Mar 2020 & 0.9 & 1.2 & Phot. & Dark & 1.53 - 1.68 & 2806\\
\hline
\end{tabular}

\begin{tablenotes}%[para,flushleft]
    \begin{flushleft}
        \small
        \textbf{Notes.} Airmass column indicates starting - final airmass of science objects.
    \end{flushleft}
\end{tablenotes}

\end{table*}

==> AA_Tables/log_MOS1_v0.tex <==
\begin{table*}
\caption{MOS1 observing log.}
\centering
\begin{tabular}{cccccc}
\hline
\hline
\begin{tabular}[c]{@{}c@{}} Observing \\ block \end{tabular} &
Date & Seeing ('') & Transparency & Moon & Airmass \\
\hline
OB01 (pre-image) & 2 Apr 2014 & 0.8 - 1.0 & Clear & Grey & 1.29 \\
OB02 & 16 Jan 2015 & 1.2 & Clear & Dark & 1.20 \\
OB03 & 3 May 2014 & 1.1 & Photometric & Dark & 1.24 \\
OB04 & 3 May 2014 & 1.2 & Photometric & Dark & 1.37 \\
OB05 & 4 May 2014 & 0.9 & Clear & Grey & 1.57 \\
OB06 & 5 May 2014 & 1.0 & Clear & Grey & 1.27 \\
OB07 & 5 May 2014 & 1.0 & Clear & Grey & 1.42 \\
OB08 & 5 May 2014 & 0.9 & Clouds & Grey & 1.72 \\
OB09 & 6 May 2014 & 1.0 & Clear & Grey & 1.29 \\
OB10 & 16 Jan 2015 & 1.0 & Clear & Dark & 1.26 \\
OB11 & 16 Jan 2015 & 0.9 & Clear & Dark & 1.39 \\
OB12 & 18 Jan 2015 & 1.1 & Clear & Dark & 1.20 \\
OB13 & 18 Jan 2015 & 0.8 & Clear & Dark & 1.25 \\
OB14 & 18 Jan 2015 & 0.8 & Clear & Dark & 1.39 \\ 
\hline
\end{tabular}
\label{table:mos1_log}
\end{table*}


==> AA_Tables/log_MOS2_v0.tex <==
\begin{table*}
\centering
\caption{MOS2 observing log.}
\label{table:mos2_log}
%\begin{threeparttable}
\begin{tabular}{cccccc}
\hline
\hline
\begin{tabular}[c]{@{}c@{}} Observing \\ block \end{tabular}  &
Date & Seeing ('') & Transparency & Moon & Airmass \\
\hline
Night-1 & 16 Feb 2018 & 0.9 & Clear & Dark & 1.34 - 1.20 - 1.36 \\
Night-2 & 17 Feb 2018 & 1.2 & Clear & Dark & 1.33 - 1.20 - 1.21 \\
\hline
\end{tabular}

\begin{tablenotes}%[para,flushleft]
    \begin{flushleft}
        \small
        \textbf{Notes.} Last column indicates starting - zenith - final airmass of science objects.
    \end{flushleft}
\end{tablenotes}

\end{table*}

==> AA_Tables/log_MOS2_v1.tex <==
\begin{table*}
\centering
\caption{MOS2 observing log.}
\label{table:mos2_log}
%\begin{threeparttable}
\begin{tabular}{ccccccc}
\hline
\hline
\begin{tabular}[c]{@{}c@{}} Observing \\ block \end{tabular}  &
Date & Seeing ('') & Transparency & Moon & Airmass & Exposure time (s)\\
\hline
Night-1 & 16 Feb 2018 & 0.9 & Clear & Dark & 1.34 - 1.20 - 1.36 & 12600 \\
Night-2 & 17 Feb 2018 & 1.2 & Clear & Dark & 1.33 - 1.20 - 1.21 & 9000 \\
\hline
\end{tabular}

\begin{tablenotes}%[para,flushleft]
    \begin{flushleft}
        \small
        \textbf{Notes.} Last column indicates starting - zenith - final airmass of science objects.
    \end{flushleft}
\end{tablenotes}

\end{table*}

